Practical Program Repair via Bytecode Mutation

Software debugging is tedious, time-consuming, and even error-prone by itself. So, various automated debugging techniques have been proposed in the literature to facilitate the debugging process. Automated Program Repair (APR) is one of the most recent advances in automated debugging, and can directly produce patches for buggy programs with minimal human intervention. Although various advanced APR techniques (including those that are either search-based or semantic-based) have been proposed, the simplistic mutation-based APR technique, which simply uses pre-defined mutation operators (e.g., changing a>=b into a>b) to mutate programs for finding patches, has not yet been thoroughly studied. In this paper, we implement the first practical bytecode-level APR technique, PraPR, and present the first extensive study on fixing real-world bugs (e.g., Defects4J bugs) using bytecode mutation. The experimental results show that surprisingly even PraPR with only the basic traditional mutators can produce genuine patches for 18 bugs. Furthermore, with our augmented mutators, PraPR is able to produce genuine patches for 43 bugs, significantly outperforming state-of-the-art APR. It is also an order of magnitude faster, indicating a promising future for bytecode-mutation-based APR.

==> figures/visAnalysis.tex <==
\begin{figure}
%\small
\scalebox{1.0}{
\begin{tabular}{rcl}
\hline 
$\vlentry(n)$&$=$&$\bigcup_{(m,n)\in E}\vlexit(m)$\\
$\vlexit(n)$&$=$&$\gen(n)\cup (\vlentry(n)-\killl(n))$\\
&&\\
$\gen(n)$&=&$\{v\mid v\in V\wedge \pi_1\circ R(v)=n\}$\\
$\killl(n)$&=&$\{v\mid v\in V\wedge \pi_2\circ R(v)=n\}$\\
\hline
\end{tabular}}
\caption{\label{fig:visibility}Static analysis for computing visibility information}
\end{figure}


==> sections/effectiveness_of_mupr.tex <==
\section{\RQOne: Effectiveness of Mutation-based Program Repair}
In this section, we answer the first research question by presenting
the number of mutants that could be considered as fixes. As noted
earlier, we are following a test case-based approach, meaning that
we take a mutant as a fix if it passes all of the test cases. Since
mutation-based program repair does an exhaustive search, it may
produce large number of mutants that pass the test-suite at hand but
do not neccessarily generalize. We call this class of mutants
\emph{plausible fixes}, while those that are semantically equivalent
to programmer-written fixes are called \emph{genuine fixes}. It is
worth noting that we consider a patch as genuine if it is syntactically
identical to the programmer-written patch or they are semantically
equivalent in an obvious way. In this section, we also present the
number of correct fixes.

Table \ref{tab:PlausibleFixesOriginal} lists all Defects4J programs
together with the number of plausible fixes for each bug of the
programs. The column \textbf{BugID} presents the identifier number
for the fixed bugs of the corresponding programs mentioned in the
column \textbf{Sub.}. The column \textbf{Time} under
\textbf{Original Mutators} and \textbf{All Mutators} represent the time
taken by \simpr (using a single-thread of execution) to sweep the whole
search space. The total number of candidate patches for each bug is
reported in column \textbf{\#Patch}, while the total number of
plausible patches is presented under column \textbf{\#Plau.}.
Finally, the number of genuine patches is presented in column
\textbf{\#Genu.}\Comment{We stress that all of these fixes are manually
checked to make sure that they indeed pass of the test cases
shipped with each program.}

As it can be seen, for \Closure we have plausible fixes for 61 versions,
but compared to the number of plausible fixes for the other benchmark
programs, the number of plausible fixes for each version of \Closure
is smaller. We attribute this phenomenon to the high coverage test suite
that is provided for this program. On the other hand, for other programs,
e.g \Chart, sometimes we end up with too many plausible fixes that none
of them are semantically equivalent to the programmer written fixes.

\input{tables/tabPlausibleFixesOriginal}

According to our definition of genuine fixes, in order to determine if a
mutant can be considered as a genuine fix, we have to compare it to the
programmer-written fix. But, deciding semantic equivalence of two programs
(in this case, a mutant of a buggy program and its fix) is, in general,
impossible. Therefore, we cannot automate this task and we had to manually
check them. Even though did not analyze the mutants and fixes deeply
(we did a syntactic check and accepted the most obvious sematically
equivalent cases), surprisingly, we found a remarkable number of
plausible fixes that can be considered as genuine fixes. Table
\ref{tab:GenuineFixesOriginal} gives a statistics about the number of
genuine fixes that we could find using default mutators of \pit.

In most cases, the defects were due to simple, single-pointed syntactic
errors. Here we present a few of the most interesting cases.
Figure \ref{fig:OverrideError:left} shows a method in version 46 of
\Closure that should not have been overridden. Programmer-written fix
simply removes the overriding method, letting the default implementation
of the method to be inherited by the enclosing class. Figure
\ref{fig:OverrideError:right} shows a mutant that achieves the same goal
by simply removing the conditional surrounding a call to the original
implementation of the method. Figure \ref{fig:RemoveSnippet:left} shows
a programmer-written fix for version 10 of \Lang that removes an \texttt{if}
statement and an unused local variable. Since the local variable is not used
elsewhere, the mutant shown in Figure \ref{fig:RemoveSnippet:right}, which
removes the same \texttt{if} statement, is going to have the same effect
(this is an example of the case where semantic equivalence is obvious). An
erroneous \texttt{return} statement in version 19 of \Time is shown in
Figure \ref{fig:ReturnVal:left}. The fix is identical to the mutation given
in Figure \ref{fig:RetrunVal:right}.

\input{tables/tabGenuineFixesOriginal}

\input{figures/errorsFixesAndMutants}

For each benchmark program, we have measured how much time does it take,
in average, to find the first plausible fix when using original mutation
operators of PIT. Table \ref{tab:timingOriginal} presents this timing
information. As it can be seen from the table, boosting the speed of \pit
has been effective as the maximum amount of time taken for finding the
first fix has become up to 3 times smaller.

\input{tables/tabTimingOriginal} 

\input{tables/tabOldRanks}

==> sections/enlarging_search_space.tex <==
\Comment{\section{\RQThree: Improving Effectiveness of Mutation-based Program Repair}
We have enlarged the search space of \simpr by the underlying mutation engine
by designing nine new mutators. These mutators are obtained by manually
inspecting a large collection of buggy Java programs, including \defectsj
programs. The mutators are designed to be general enough so that they can be
used in fixing as many programs as possible. Note that these new mutators are
still operating in the bytecode level, but for the sake of simplicity in
presentation we have described them in Java source code level. In what follows,
$P\lbrack e\rbrack$ represent a Java program with single placeholder in it which
is instantiated with a program element $e$. Furthermore,
$P\lbrack e\rbrack\hookrightarrow P\lbrack e'\rbrack$ represents a rewrite rule
that mutates $e$ to $e'$ while leaving the rest of the program unchanged. Lastly,
we use set membership notation to represent the fact that a class, a method, or a
field is declared inside some type, and also use ellipsis to show the portions of
the program that are inconsequential.
\paragraph{METHOD\_CALL\_GUARD\_MUTATOR} Mutates a non-void method call to check if the argument pointing to the receiver object is \texttt{null} to return the default value \cite{bib:GJSGGB14} corresponding to the return type of the callee method. Otherwise, the result of the method call is returned. More precisely,
\begin{equation}\label{rule:METHCALLGUARDMUTATOR}
  \ruledef{\begin{matrix}
    \mathtt{T~meth()\{\dots\}}\in \mathtt{C} \\
    \mathtt{T}\neq\mathtt{void}\qquad \mathtt{v}:\mathtt{C} \\
    def~\text{is the default value of}~\mathtt{T}
\end{matrix}}{P\lbrack \mathtt{v.meth()}\rbrack\hookrightarrow P\lbrack \mathtt{(v == null~}\text{\texttt{?}}~def~\mathtt{:~v.meth())}\rbrack}
\end{equation}
\paragraph{FIELD\_ACCESS\_MUTATOR} Replaces an accesses to a field with an access to another field provided that the other field is visible in the context. More concretely,
\begin{equation}\label{rule:FIELDACCESSMUTATOR}
  \ruledef{\begin{matrix}
             \mathtt{\dots~\{\dots v.f\dots\}}\in\mathtt{S}\\
             \mathtt{v:C}\qquad\mathtt{T~f}\in\mathtt{C}\qquad\mathtt{f}\neq\mathtt{g}\\
             \mathtt{C}\neq\mathtt{T}\implies visible(\mathtt{g}, \mathtt{C}, \mathtt{S})\\
             static(\mathtt{f}, \texttt{C})\implies static(\mathtt{g}, \texttt{C})
           \end{matrix}}{P\lbrack \mathtt{v.f}\rbrack\hookrightarrow P\lbrack \mathtt{v.g}\rbrack}
\end{equation}
where $visible(\mathtt{g}, \mathtt{C}, \mathtt{S})$ holds if and only if \texttt{g} is declared to be \texttt{public} in \texttt{C} or \texttt{C}, \texttt{S} are in the same package (or  and \texttt{S}  \texttt{C}\texttt{g} is declared to be \texttt{protected}
\begin{itemize}
  \item METHOD\_CALL\_MUTATOR: replaces a method call of the form \texttt{o.meth1(...)} with \texttt{o.meth2(...)}, where \texttt{meth1}, \texttt{meth2} have the same signature and a value of \texttt{meth2}'s return type is expected by the context. The methods have to be declared in the same class, and \texttt{meth2} should be visible. The mutator also works on static methods. If there is no such \texttt{meth2}, the code is left unmutated.
  \item LOCAL\_MUTATOR: replaces a use of a local variable \texttt{a} with a use of another visible local variable \texttt{b} such that a value of \texttt{b}'s type is expected by the context. If there is no such \texttt{b}, the code is left unmutated.
  \item NULLNESS\_CHECK\_SAME\_LOCAL: upon a use of a reference-typed local variable \texttt{v}, the mutator inserts a conditional to check if \texttt{v == null}. If it is the case, the mutated code returns the value of some local variable visible at the point. The local variable should have the same type as the return type of the mutated method. If there is no visible variable of the appropriate type, the code is left unmutated. Furthermore, if the method returns \texttt{void}, the mutated code simply exits from the method.
\end{itemize}
Table \ref{tab:newPlausibleGenuine} shows the result of applying these new mutators on \defectsj programs, in terms of the number of plausible and genuine fixes obtained. In this table, as before, the column \textbf{Fixing} represents the number of plausible fixes, while \textbf{Genuine} reports the number of genuine fixes. The last column, shows the ratio of total number of bugs that are genuinely fixed over the total number of bugs that are fixes.
\input{tables/tabNewPlausibleGenuine}
\input{tables/tabNewRanks}}

==> sections/helping_manual_debugging.tex <==
\Comment{\section{\RQTwo: Helping With Manual Debugging}
Even though we cannot always categorize mutants that pass all the
test cases as genuine, in most cases they give hints that can help programmers with manual debugging. The usefulness of the hint can be estimated by its relevance to the bug. We estimate this relevance according to different metrics such as closeness of the mutation point to the buggy code or degree of dependence of the buggy code to the mutated statement. We use the symbols introduced in Table \ref{tab:QualityLegend} to represent the usefulness of a hint.

\input{tables/tabQualityLegend.tex}

Table \ref{tab:hintsOriginal} presents the number of mutants that fall into each category. In what follows, we are going to give an example from each category. When debugging a large program, localizing the bug-inducing statement(s) is of particular importance. This will save much time and even helps someone who is not familiar with the code base to fix the bug within a reasonable amount of time. For example, bug number 25 of \Chart is located inside the methods \texttt{drawHorizontalItem} and \texttt{drawVerticalItem}. The actual fix involves addition and modification of several lines of code in the body of the methods. The mutation, however, take place inside the method \texttt{getMeanValue} of the class \texttt{Default\-Statistical\-Category\-Dataset}. The mutation turns the method into a constant function by making it to return \texttt{null} each time it is called. This affects control-flow inside a top-level method that calls the buggy methods.

\input{tables/tabHintsOriginal.tex}

In a well-written object-oriented program, methods are usually small in size, so mutating a buggy method that passes all the test cases gives good hint about the location of the actual bug. Also mutations that directly remove the call to a buggy method give a decent hint about the fix. For example, there is another mutation that also fixes the bug number 25 of \Chart but its quality is higher than the one described in the previous paragraph in that it fixes the program by removing an \texttt{if}-statement that leads to the calls to the two buggy methods.

Another class of mutations happen to be located right on the location that actual fix is applied. Bug number 17 of \Time is located inside the method \texttt{adjustOffset} of the class \texttt{DateTimeZone}. The actual fix involves addition of several new lines of code. It also modifies three lines of buggy codes. Our mutation produces one of these lines by replacing the call to the method \texttt{convert\-UTC\-To\-Local} with its argument.}

==> sections/related_work.tex <==
\section{Related Work}\label{sec:RelatedWork}
At the top level, based on the actions they take for repairing
programs, \apr techniques can be categorized into two classes: (1)
runtime (dynamic) healing techniques; (2) code fixing
technique. Runtime healing techniques seek to detect and recover
erroneous state while the program is running. These techniques are
sound (i.e. they change the program behavior when it is indeed
necessary), and can be effectively applied on software whose source code
is not available. Runtime overhead is the primary disadvantage of
dynamic healing techniques. ClearView \cite{bib:PKLABCPSSSWZER09} and
RCV \cite{bib:LDR14} are two well-known dynamic healing technique. The
second category is the most relevant to the present work. In what
follows, we review the most related work in this category. We stress
that this review is by no means complete and, for a better
appreciation of the effectiveness of our technique, we invite the
reader to consult the latest survey papers \cite{bib:GMM17,bib:Monp18}
in this field.

\subsection{Search-based \apr}
Search-based techniques, as the name suggests, search through the
search space of possible fixes. For each candidate fix, they modify
the source code of the program and test it against the set of available test cases. This implies that search-based techniques completely fall into the bigger category of generate-and-validate techniques. Search-based techniques differ from each other in the way they search through the space of possible
fixes. In what follows, we briefly discuss the most recent work in this category.\Comment{In this respect, they can be further classified into three
subcategories\lingming{there are actually five paragraphs after this paragraph, you want to condense the text and have three paragraphs
  for three categories. Normally, you only need one to three sentences
  to discuss a normal work, you may need more for closely related work
  (e.g., mutation ones). It is also better to put mutation one in the
  last position since it's most related to this work}}

To the best of our knowledge, the work by Debroy and Wong \cite{bib:DW10} is the first and the only serious activity devoted on mutation-based program repair. They build a mutation engine for both C and Java, and report the number of generated and fixing mutants. This first attempt, has several shortcomings, though: (1) they do not examine each fixing mutant to see if the mutant is indeed a genuine fix; (2) studied benchmark programs are small and limited; (3) a limited number of mutation operators have been studied; (4) it is not clear how efficient is their technique. Despite using a small set of hand-picked (single-fault) benchmark programs, they have been able to fix at most 34.78\% of the bugs. In fact, thanks to a recent (faithful) implementation of this technique \cite{bib:MM16}, we realized that it falls short of repairing bugs in large, realistic programs.\Comment{ The reason is that the set of mutation operators employed by the tool is very limited. What we need is more mutation operators and, more importantly, an efficient way of generating and validating mutants (otherwise, employing a large set of mutation operators would not be practical).} Compared to the previous work in this sub-category, our work is novel in that we study a diverse set of mutation operators.\Comment{ This has been possible because we work on bytecode level (as opposed to source code level), and also take advantage of parallelism, enabling us to generate and validate tens of mutants per second.} Furthermore, we analyze each mutant deeply to decide if it is a genuine fix or give any hints about fixing the program. Thereby presenting a clearer picture of effectiveness of mutation-based program repair.

Another category of APR techniques use Evolutionary Computation methods, such as Genetic Programming (GP), to evolve a buggy program to one that passes all the available test cases. In their paper \cite{bib:WNGF09}, Weimer et al. studied GP-based program repair for the first time. Later, they employed the technique in a mature APR tool for C, called GenProg \cite{bib:GNFW12}.\Comment{ As part of an extended form of GP, GenProg incorporates several mutation operators (at the statement level), and the idea of looking for fix ingredients from other parts of the same program (an idea that have later been studied thoroughly under the name of \emph{plastic surgery} hypothesis \cite{bib:BBDHS14}). After finding a variant that passes all the test cases, GenProg uses delta-debugging to prune redundant parts of the variant, making it more human-readable.} We believe GenProg has been very successful, but it still suffers from at least two problems: (1) it works at the \emph{statement-level} AST making it miss many fix opportunities; (2) it is not computationally (also space-wise) efficient, as working on source code level implies the need for complicated, language-dependent AST processing and recompilation for each generated variant. A recent research \cite{bib:WCWHC18}, addresses the first problem by working on \emph{expression-level} AST. Regarding the second problem of GenProg, in a subsequent paper \cite{bib:GVFW12}, Le Goues et al. argue that the benefit from using GenProg worth using expensive, powerful computing infrastructures.

Unfortunately, it seems that the developers of GenProg were oblivious about the overfitting problem inherent to generate-and-validate techniques. In fact, a subsequent study \cite{bib:QLAR15} shows that only a small fraction of fixes produced by GenProg could be considered genuine fixes. Another study \cite{bib:QMLDZW14} shows that, in general, GenProg does not perform better than random search, posing doubt on the rationale of using rather complicated algorithms employed in GenProg. Furthermore, comparing jGenProg \cite{bib:MM16}, a faithful implementation of GenProg for Java, to a basic mutation-based program repair technique discussed early in this section demonstrates that the difference between the number of fixes produced by GenProg and the mutation-based technique, in the cases where GenProg performed better, is small.

SPR (Staged Program Repair) \cite{bib:LR15}, and its successor Prophet \cite{bib:LR16b}, are two examples of the most precise generate-and-validate tools available. SPR defines a set of operators that ultimately help filtering out many variants that cannot pass the existing test cases. This results in a more focused search of the search space. Prophet attempts to elaborate Staged Program Repair in terms of speed and precision by learning from a collection of past commits. Though showing promising results, SPR and Prophet are both quite slow. Furthermore, they target only C programming language.

CapGen \cite{bib:WCWHC18} is the most recent searched-based APR technique that is very similar to GenProg. In fact, it addresses the precision deficiency of GenProg by working at an expression-level AST. In order to cope with the enlarged search space, it takes advantage of ``context'' information to prioritize both fix ingredients. Type information, such as expected type in a context, together with the type of the expression to be synthesized or grafted in the context, happen to provide useful context information so as to prioritize fix ingredients based their likelihood of leading to plausible and genuine patches. It also takes advantage of the statistical results from past work to heuristically prioritize fix operations. CapGen has been evaluated on a subset of Defects4J programs showing that the tool, except for a few cases, runs fast and can produce quite a few genuine fixes. The problem with CapGen is that the ranks of generated plausible fixes, that turn out to be genuine fixes, are usually far more than 10 making it difficult to get help from this tool. Furthermore, the tool does not show a predictable running time behavior; for example, it takes only 11 seconds to fix a large program, while it takes more than 50 minutes to fix a smaller program.

\subsection{Semantic-based \apr}
AutoFix \cite{bib:PFNWMZ14} uses contracts (pre- and post-conditions)
to provide high quality fix suggestions, and also automate the whole
repair process. Contracts enhance the precision of fault detection,
fault localization, and validating fixes by providing a specification
of correct behavior. AutoFix requires modest programmer annotation
burden (Eiffel programmers usually provide pre- and post-condition
specifications on a daily basis); the only required user input to the
AutoFix supporting tool is just a faulty program annotated with
contracts. The tool produces a collection of validated fixes for the
fault ranked according to an estimate of their suitability. JAID
\cite{bib:LPF17} is an implementation of AutoFix for Java. Even though
Java lacks language constructs for specifying contracts, JAID infers
predicates that can be used as contracts, thereby directly using
techniques employed by AutoFix. Angelix \cite{bib:MYR16} and semfix
\cite{bib:MYR16} are two other highly cited semantic-based APR
tools. \lingming{we should discuss the brief idea of each technique (one to
three sentences each), rather than having long description for autoFix but
no description for angelix and semfix.}

%mutation testing history, list all the works on mutation testing, including various applications of mutation testing. State the importance of our work(first large scale study on mutation-based program repair, and demonstrate the practicability of mutation-based repair, say fixing over 30 bugs!!).

%program repair history, list all works on program repair. State the difference between this and prior work (e.g., mutation-based, bytecode-level, release maven plugin (one-command fix doable!), we can fix the most bugs!!)


==> sections/research_questions.tex <==
\section{Research Questions}\label{sec:RQs}
We are going to answer the following research questions.
\begin{enumerate}
    \item[\RQOne] How does mutation testing help with automatic program repair on real bugs? %effectiveness and efficiency; also report genuine fixes
    \item[\RQTwo] How does mutation testing help with manual program repair? %give some hint to the programmer; summarize 4 or 5 different case that mutation testing give hint--> directly at the patch location or somewhere deep in the call stack.
%  \item How effective is mutation-based program repair?
% practical aspects:
    \item[\RQThree] How to improve effectiveness of program repair? % Which mutation operators are most effective in repair? Does enlarging search space improve effectiveness of the technique?
    \item[\RQFour] How can we do even faster mutation based program repair? %prioritize statements based on e.g Ochiai and mutator type. E.g. stop testing mutants after first observed failed test case
\end{enumerate} 

==> tables/tabGenuineFixesOriginal.tex <==
\begin{table}
  \centering
  \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{ID} & \textbf{Bug No.} & \textbf{Genuine} & \textbf{Fixed Bugs} \\ \hline \hline
    \Chart & 1 & 1 & 1 \\ \hline
    \multirow{2}{*}{\Time} & 11 & 1 & \multirow{2}{*}{2} \\
    & 19 & 2 & \\ \hline
    \Lang & 10 & 2 & 1 \\ \hline
    \multirow{4}{*}{\Math} & 50 & 1 & \multirow{4}{*}{4} \\
    & 65 & 1 & \\
    & 82 & 1 & \\
    & 85 & 1 & \\ \hline
    \multirow{11}{*}{\Closure} & 11 & 4 & \multirow{11}{*}{11} \\
    & 21 & 3 & \\
    & 31 & 1 & \\
    & 40 & 1 & \\
    & 46 & 2 & \\
    & 62 & 1 & \\
    & 63 & 1 & \\
    & 70 & 1 & \\
    & 73 & 1 & \\
    & 86 & 2 & \\
    & 126 & 2 & \\
    \hline
  \end{tabular}
  \caption{Summary of genuine fixes when applying original mutators of PIT}\label{tab:GenuineFixesOriginal}
\end{table} 

==> tables/tabHintsOriginal.tex <==
\begin{table}
  \centering
  \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{ID} & \textbf{+} & \textbf{++} & \textbf{+++}\\ \hline
    \hline
    \Chart & 5 & 12 & 7 \\
    \Time & 4 & 1 & 2 \\
    \Mockito & 0 & 3 & 1 \\
    \Lang & 3 & 0 & 20 \\
    \Math & 11 & 83 & 24 \\
    \Closure & 7 & 13 & 19 \\
    \hline
  \end{tabular}
  \caption{Number of hints from each quality category when applying original mutators of PIT (genuine fixes are excluded)}\label{tab:hintsOriginal}
\end{table} 

==> tables/tabNewPlausibleGenuine.tex <==
\begin{table}
  \centering
  \begin{scriptsize}
  \begin{tabular}{|c|c|c|c|c|}
    \hline
    \textbf{ID} & \textbf{Bug No.} & \textbf{Fixing} & \textbf{Genuine} & \textbf{Ratio} \\ \hline \hline
    \multirow{9}{*}{\Chart} & 3 & 1 & 0 & \multirow{9}{*}{4/9} \\
    & 4 & 1 & 1 & \\
    & 5* & 1 & 0 & \\
    & 7 & 4 & 0 & \\
    & 11 & 2 & 2 & \\
    & 13* & 2 & 0 & \\
    & 24 & 1 & 1 & \\
    & 25* & 59 & 0 & \\
    & 26* & 30 & 2 & \\ \hline
    \multirow{4}{*}{\Time} & 4* & 1 & 0 & \multirow{4}{*}{0/4} \\
    & 7 & 1 & 0 & \\
    & 11* & 4 & 0 & \\
    & 20 & 3 & 0 & \\ \hline
    \multirow{3}{*}{\Mockito} & 8* & 2 & 0 & \multirow{3}{*}{2/3} \\
    & 29 & 1 & 1 & \\
    & 38 & 1 & 1 & \\ \hline
    \multirow{9}{*}{\Lang} & 6 & 1 & 1 & \multirow{9}{*}{3/9} \\
    & 7 & 3 & 0 & \\
    & 10* & 1 & 0 & \\
    & 22* & 1 & 0 & \\
    & 25 & 1 & 0 & \\
    & 27* & 1 & 0 & \\
    & 33 & 1 & 1 & \\
    & 39* & 5 & 0 & \\
    & 59 & 1 & 1 & \\ \hline
    \multirow{4}{*}{\Math} & 33 & 1 & 1 & \multirow{4}{*}{3/4} \\
    & 39* & 5 & 0 & \\
    & 59 & 1 & 1 & \\
    & 75 & 1 & 1 & \\ \hline
    \multirow{26}{*}{\Closure} & 7* & 2 & 0 & \multirow{26}{*}{6/26} \\
    & 8* & 1 & 0 & \\
    & 10* & 1 & 1 & \\
    & 11** & 7 & 6 & \\
    & 12* & 1 & 0 & \\
    & 14 & 1 & 1 & \\
    & 15* & 1 & 0 & \\
    & 17* & 2 & 0 & \\
    & 21* & 5 & 0 & \\
    & 22 & 1 & 0 & \\
    & 29 & 1 & 0 & \\
    & 30* & 1 & 0 & \\
    & 33* & 1 & 0 & \\
    & 35 & 1 & 0 & \\
    & 36* & 2 & 0 & \\
    & 45* & 4 & 0 & \\
    & 46** & 4 & 2 & \\
    & 48* & 3 & 0 & \\
    & 50* & 1 & 0 & \\
    & 59* & 2 & 0 & \\
    & 66* & 1 & 0 & \\
    & 72* & 1 & 0 & \\
    & 76* & 1 & 0 & \\
    & 78 & 1 & 0 & \\
    & 92* & 1 & 1 & \\
    & 93* & 1 & 1 & \\
    \hline
  \end{tabular}
  \end{scriptsize}
  \caption{Summary of fixes when applying our five new mutators} \label{tab:newPlausibleGenuine}
\end{table} 

==> tables/tabNewRanks.tex <==
\begin{table}
  \centering
  \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{ID} & \textbf{Bug No.} & \textbf{Plausibles} & \textbf{Search Space} \\ \hline \hline
    \multirow{4}{*}{\Chart} & 4 & 1 & 30 \\
    %& 7 & 4 & 127 \\
    & 11 & 2 & 22 \\
    & 24 & 1 & 2 \\
    & 26 & 2 & 268 \\ \hline
    \multirow{2}{*}{\Mockito} & 29 & 1 & 1 \\
    & 38 & 1 & 1 \\ \hline
    \multirow{3}{*}{\Lang} & 6 & 1 & 49 \\
    & 33 & 1 & 1 \\
    & 59 & 1 & 1 \\ \hline
    \multirow{3}{*}{\Math} & 33 & 1 & 1 \\
    & 59 & 1 & 1 \\
    & 75 & 1 & 1 \\ \hline
    \multirow{6}{*}{\Closure} & 10 & 1 & 850 \\
    & 11 & 7 & 2407 \\
    & 14 & 1 & 1 \\
    & 46 & 2 & 27 \\
    & 92 & 1 & 38 \\
    & 93 & 1 & 38 \\
    \hline
  \end{tabular}
  \caption{Ranking of the genuine fixes among other plausible fixes and also among the whole search space, when applying new mutators}\label{tab:newRanks}
\end{table}


==> tables/tabOldRanks.tex <==
\begin{table}
  \centering
  \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{ID} & \textbf {Bug No.} & \textbf{Plausibles} & \textbf{Search Space}\\ \hline \hline
    \Chart & 1 & 2 & 52 \\ \hline
    %& 13 & 5 & 146 \\ \hline
    \multirow{2}{*}{\Time} & 11 & 2 & 30 \\
    & 19 & 2 & 921 \\ \hline
    %} & 7 & 2 & 223 \\
    \Lang & 10 & 1 & 206 \\ \hline
    \multirow{4}{*}{\Math} & 50 & 5 & 14 \\
    & 65 & 1 & 15 \\
    %& 81 & 4 & 23 \\
    & 82 & 3 & 145 \\
    & 85 & 1 & 164 \\ \hline
    \multirow{11}{*}{\Closure} & 11 & 4 & 2087 \\
    & 21 & 4 & 10 \\
    & 31 & 1 & 5011 \\
    & 40 & 1 & 25 \\
    & 46 & 2 & 20 \\
    & 62 & 1 & 8 \\
    & 63 & 1 & 8 \\
    & 70 & 1 & 1 \\
    & 73 & 1 & 38 \\
    & 86 & 2 & 2 \\
    & 126 & 1 & 1 \\
    \hline
  \end{tabular}
  \caption{Ranking of the genuine fixes among other plausible fixes and also among the whole search space, when applying original PIT mutators}\label{tab:oldRanks}
\end{table} 

==> tables/tabPlausibleFixesOriginal.tex <==
\begin{table}
  \centering
  \begin{scriptsize}
  \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{ID} & \textbf{Bug No.} & \textbf{Fixing} & \textbf{Fixed Bugs} \\ \hline \hline
    \multirow{7}{*}{\Chart} & 1 & 2 & \multirow{7}{*}{7} \\
    & 5 & 1 & \\
    & 12 & 1 & \\
    & 13 & 7 & \\
    & 15 & 1 & \\
    & 25 & 104 & \\
    & 26 & 34 & \\ \hline
    \multirow{5}{*}{\Time} & 4 & 3 & \multirow{5}{*}{5} \\
    & 11 & 29 & \\
    & 17 & 2 & \\
    & 19 & 2 & \\
    & 24 & 3 & \\ \hline
    \Mockito & 8 & 4 & 1 \\ \hline
    \multirow{11}{*}{\Lang} & 7 & 2 & \multirow{11}{*}{11} \\
    & 10 & 2 & \\
    & 22 & 1 & \\
    & 27 & 5 & \\
    & 31 & 1 & \\
    & 39 & 3 & \\
    & 43 & 2 & \\
    & 44 & 2 & \\
    & 51 & 2 & \\
    & 58 & 1 & \\
    & 63 & 6 & \\ \hline
    \multirow{23}{*}{\Math} & 2 & 15 & \multirow{23}{*}{23} \\
    & 6 & 1 & \\
    & 8 & 5 & \\
    & 20 & 20 & \\
    & 28 & 27 & \\
    & 29 & 2 & \\
    & 32 & 3 & \\
    & 39 & 2 & \\
    & 49 & 5 & \\
    & 50 & 5 & \\
    & 57 & 1 & \\
    & 63 & 6 & \\
    & 65 & 1 & \\
    & 71 & 4 & \\
    & 78 & 2 & \\
    & 80 & 11 & \\
    & 81 & 26 & \\
    & 82 & 3 & \\
    & 84 & 3 & \\
    & 85 & 4 & \\
    & 88 & 1 & \\
    & 95 & 3 & \\
    & 104 & 1 & \\ \hline
    \multirow{38}{*}{\Closure} & 5 & 1 & \multirow{38}{*}{38} \\
    & 7 & 2 & \\
    & 8 & 2 & \\
    & 10 & 2 & \\
    & 11 & 5 & \\
    & 12 & 3 & \\
    & 13 & 7 & \\
    & 15 & 1 & \\
    & 17 & 1 & \\
    & 21 & 10 & \\
    & 30 & 1 & \\
    & 31 & 1 & \\
    & 33 & 1 & \\
    & 36 & 4 & \\
    & 38 & 1 & \\
    & 40 & 2 & \\
    & 42 & 2 & \\
    & 45 & 4 & \\
    & 46 & 3 & \\
    & 48 & 3 & \\
    & 50 & 2 & \\
    & 59 & 1 & \\
    & 62 & 2 & \\
    & 63 & 2 & \\
    & 64 & 1 & \\
    & 66 & 2 & \\
    & 68 & 1 & \\
    & 70 & 1 & \\
    & 72 & 1 & \\
    & 73 & 1 & \\
    & 76 & 2 & \\
    & 81 & 2 & \\
    & 84 & 2 & \\
    & 86 & 2 & \\
    & 92 & 2 & \\
    & 93 & 2 & \\
    & 101 & 2 & \\
    & 126 & 2 & \\
    \hline
  \end{tabular}
  \end{scriptsize}
  \caption{Summary of plausible fixes when applying original mutators of PIT}\label{tab:PlausibleFixesOriginal}
\end{table} 

==> tables/tabQualityLegend.tex <==
\begin{table}
  \centering
    \begin{tabularx}{\linewidth}{|c|X|}
      \hline
      \textbf{Quality} & \textbf{Description} \\ \hline
      \hline
      + & The mutation gives a slight hint about the location/cause of the bug. The mutation removes a call to a method which calls the buggy method, or at least one statement is control/data dependent \cite{bib:Much97} on the mutated statement. \\ \hline
      ++ & The mutation gives a stronger hint about the location/cause of the bug. The mutated and the buggy statement reside in the same method, the mutation removes the invocation of a buggy method, or at least one buggy statement is control/data dependent on the mutated statement. \\ \hline
      +++ & The mutation exactly locates the buggy statement and/or partially generates a genuine fix. \\
      \hline
    \end{tabularx}
  \caption{Symbols that we use to classify plausible fixes based on the quality of hints they provide for manual debugging }\label{tab:QualityLegend}
\end{table} 

==> tables/tabTimingOriginal.tex <==
\begin{table}
  \centering
  \begin{tabular}{|c|c|}
    \hline
    \textbf{ID} & \textbf{Time (avg)} \\ \hline
    \hline
    \Chart & 42 s \\
    \Time & 61 s \\
    \Mockito & 1 m 30 s \\
    \Lang & 26 s \\
    \Math & 6 m 24 s \\
    \Closure & 17 m 27 s \\
    \hline
  \end{tabular}
  \caption{Timing of original mutators of PIT}\label{tab:timingOriginal}
\end{table}
